Towards Better Understanding Researcher Strategies in Cross-Lingual Event Analytics

With an increasing amount of information on globally important events, there is a growing demand for efficient analytics of multilingual event-centric information. Such analytics is particularly challenging due to the large amount of content, the event dynamics and the language barrier. Although memory institutions increasingly collect event-centric Web content in different languages, very little is known about the strategies of researchers who conduct analytics of such content. In this paper we present researchers' strategies for the content, method and feature selection in the context of cross-lingual event-centric analytics observed in two case studies on multilingual Wikipedia. We discuss the influence factors for these strategies, the findings enabled by the adopted methods along with the current limitations and provide recommendations for services supporting researchers in cross-lingual event-centric analytics.

==> 05_interviews.tex <==
\section{Post-Sessions Interviews}
\label{sec:interviews}

At the end of each study, we conducted individual semi-structured interviews with the study participants to better understand their views on the different aspects of the analysis processes. 
In particular, the interviews included questions regarding the relevance of event-centric research in Wikipedia, the scope of the study, 
as well as the main findings from their perspective.
Furthermore, we requested the participant feedback with respect to the tools they used and asked for desired functionalities not supported yet. 

\textbf{Relevance of event-centric research in Wikipedia:}
The participants of both studies characterized the relevance of research on the respective events by their impact at the study time, and the novelty of the studies conducted close to the event dates.
%
From the sociological perspective, the mutual influence between the article development and the important events in the society has also been mentioned as an important research aspect. 

\textbf{The scope of the study:}
Both studies differed in their goals, leading to differences in the scope of the analyzed data collections. 

In \brexit{}, the participants focused on the temporal dimension of the event and quickly narrowed down the scope of the study to the specific articles to facilitate in-depth analysis. 
%
For the participants with sociology background, rich discussions that occurred in Wikipedia as related articles emerged were of particular interest.

In contrast, in \paris{}, the participants emphasized their goal to better understand the coverage of the event. Therefore, they aimed to collect a possibly complete set of articles across all languages mentioning the US pullout. Additionally, the participants with information design background voiced their intention to analyze topically related articles that contained many images. 

\textbf{Key findings from the participant perspective:}
%
The observations of the participants cover various aspects of the event representation, such as the dynamics and neutrality of the articles, the differences in coverage across languages and, in \paris{}, the strict separation between climate and politics related articles.

In the context of dynamics, the participants compared the Wikipedia articles on Brexit with news websites due to the fast reaction of the Wikipedia editors to the event development.
%
The participants also highlighted the evolution of the article neutrality. Whereas the articles were not 
initially neutral, their neutrality improved over time with moderation support, such as locking comments during the event development.

\parisnew{In \paris{}, the participants were surprised by the differences in coverage of the US pullout across languages: while the English Wikipedia covered it in all its details, it was not mentioned anywhere in the Italian Wikipedia. 
%
Another aspect was the focus on Donald Trump: one of the participants expressed the impression that Wikipedia was rather about Trump's pullout of the Paris Agreement than a US pullout.
%
Another unexpected output was the strict separation between politics and science in Wikipedia: Only very few mentions of the US pullout were found in climate-related articles. However, the multimedia-based network analysis revealed the indirect effect of the pullout even on climate-related articles.} 

\textbf{Recommendations:} %
%
With respect to the methods and tools required to better support cross-cultural studies, the participants expressed the need for functionalities enabling to:

\begin{itemize}
\item[R1] (Content) Obtain a more generalized overview of the event as an entry point, as opposed to the direct article comparison, which is useful at a later stage (zoom out/in).

\item[R2] (Temporal) Provide a higher temporal resolution for the article revisions, including fact propagation.

\item[R3] (Network) Provide insights into the communities behind the articles.

\item[R4] (Controversy) Provide insights into the discussion pages in different languages, their similarities and differences.

\end{itemize}

